Multi-task Causal Learning with Gaussian Processes

This paper studies the problem of learning the correlation structure of a set of intervention functions defined on the directed acyclic graph (DAG) of a causal model. This is useful when we are interested in jointly learning the causal effects of interventions on different subsets of variables in a DAG, which is common in field such as healthcare or operations research. We propose the first multi-task causal Gaussian process (GP) model, which we call DAG-GP, that allows for information sharing across continuous interventions and across experiments on different variables. DAG-GP accommodates different assumptions in terms of data availability and captures the correlation between functions lying in input spaces of different dimensionality via a well-defined integral operator. We give theoretical results detailing when and how the DAG-GP model can be formulated depending on the DAG. We test both the quality of its predictions and its calibrated uncertainties. Compared to single-task models, DAG-GP achieves the best fitting performance in a variety of real and synthetic settings. In addition, it helps to select optimal interventions faster than competing approaches when used within sequential decision making frameworks, like active learning or Bayesian optimization.

==> advantages.tex <==
\subsection{Advantages of using the causal operator} \label{sec:operator}
The causal operator allows us to write any $t_s(\x)$ as an integral transformation of $\basefunction$. The integrating measure $p(\bvalue|\DO{\X_s}{\x})$, which differ across $\X_s$, captures the dependency structure between the base set and the intervention set and can be reduced to \textit{do}-free operations via \textit{do}-calculus.
Notice how, given our identifiability assumptions, all functions in $\T$ can also be computed by simply applying the rules of \textit{do}-calculus when observational data are available. However, writing the functions via $L_s(\basefunction)(\x)$ allows to:
\begin{itemize}
	\item identify the correlation structure across functions and thus specify a multi-task probabilistic model and share experimental information;
	\item learn those intervention functions for which we cannot run experiments;
	\item efficiently learn $\T$ when $\partsX$ is large and specifying a model for each $t_s(\x)$ would be computationally expensive and could lead to inconsistent prior specification across functions;
	\item model a system by only making one single assumption on $\basefunction$ which is then propagated in the \DAG;
	\item correctly quantify uncertainty within decision making frameworks.
\end{itemize}
\fig \ref{fig:dags2} (a) shows how information propagates when different experimental outputs are observed and a multi-task model is used. 
When an intervention is performed, the information is propagated in the graph through $\basefunction$ which links the different interventional functions. Using $\basefunction$ we avoid the specification of the correlation structure across every pair of intervention functions which would result in a combinatorial problem. 


%%By analogy with the causal calculus theory
%Using the terminology of \textit{do}-calculus, we can see \eq \eqref{eq:eq_theorem} as a \emph{functional} front-door adjustment formula where the set satisfying a functional front-door criterion is given by the base set $\B = (\I \cup \C)$. The set $\B$ satisfies the functional front-door criterion if the conditions in Theorem \ref{theorem_transfer} are respected. Finally, as for \textit{do}-calculus \citet{galles2013identif} give graphical conditions for the identifiability of causal effects, Theorem \ref{function_existence} gives a graphical condition for the identifiability of the causal operator and thus our multi-task causal calculus.


==> causal_operator.tex <==

%\subsection{Causal operator vs \textit{do}-calculus} \label{sec:operator}
\subsection{Advantages of using the causal operator} \label{sec:operator}
The causal operator allows us to write any $t_s(\x)$ as an integral transformation of $\basefunction$. The integrating measure $p(\bvalue|\DO{\X_s}{\x})$, which differ across $\X_s$, captures the dependency structure between the base set and the intervention set and can be reduced to \textit{do}-free operations via \textit{do}-calculus.
Notice how, given our identifiability assumptions, all functions in $\T$ can also be computed by simply applying the rules of \textit{do}-calculus when observational data are available. However, writing the functions via $L_s(\basefunction)(\x)$ allows to:
\begin{itemize}
	\item identify the correlation structure across functions and thus specify a multi-task probabilistic model and share experimental information;
	\item learn those intervention functions for which we cannot run experiments;
	\item efficiently learn $\T$ when $\partsX$ is large and specifying a model for each $t_s(\x)$ would be computationally expensive and could lead to inconsistent prior specification across functions;
	\item model a system by only making one single assumption on $\basefunction$ which is then propagated in the \DAG;
	\item correctly quantify uncertainty within decision making frameworks.
\end{itemize}
\fig \ref{fig:dags2} (a) shows how information propagates when different experimental outputs are observed and a multi-task model is used. 
When an intervention is performed, the information is propagated in the graph through $\basefunction$ which links the different interventional functions. Using $\basefunction$ we avoid the specification of the correlation structure across every pair of intervention functions which would result in a combinatorial problem. 


%%By analogy with the causal calculus theory
%Using the terminology of \textit{do}-calculus, we can see \eq \eqref{eq:eq_theorem} as a \emph{functional} front-door adjustment formula where the set satisfying a functional front-door criterion is given by the base set $\B = (\I \cup \C)$. The set $\B$ satisfies the functional front-door criterion if the conditions in Theorem \ref{theorem_transfer} are respected. Finally, as for \textit{do}-calculus \citet{galles2013identif} give graphical conditions for the identifiability of causal effects, Theorem \ref{function_existence} gives a graphical condition for the identifiability of the causal operator and thus our multi-task causal calculus.




==> discussion_experiment.tex <==
\subsection{Discussion of experiments}
Interestingly, $N$ affects the performance results in different ways. First of all, as $N$ increases, the accuracy of the conditional distributions in the \DAG improves for those interventional levels that are observed in the data. This means that, for those values, the do-estimates improve, the causal \gptext prior becomes more precise and the  estimates of the integrating measures needed for \our improve thus enhancing the transfer of information. However, the estimates of the conditional distribution might get deliberately bad for those interventional levels that are not observed in the data making the average performance across the interventional range decrease for increasing $N$. We can see this effect for $\DAG2$ and $\DAG4$ where the performance of the do-effects computation decline for $N=100$ (\tbl \ref*{table_100}). 
The benefit of having more observational data depends on their coverage of the considered interventional domains. 

In addition, through the estimates for the conditional distributions, $N$ impacts on the causal \gptext prior parameters and thus on the model predictive variance. When the do-calculus computations are less precise the model variance is inflated thus making both \al and \cbo based on $\our^+$ or $\gptext^+$ be much more explorative. For $\DAG4$, the do-effects becomes on average less exact for $N=100$ (\tbl \ref*{table_100}). The variance of the do-effects increases in this case making $\our^+$ or $\gptext^+$ collect more observations in areas where when $\dataset^O$ are not observed and thus slowing down their convergence to the minimum \rmse (\fig \ref{fig:al_bo_complete} left panel). 

Overall, our results show how, across different \DAG{s}, values of $N$, initialisation of $\dataset^I$ and prior specification, $\our$ reaches the best performances making it a robust default choice for any experiment. 

\input{advantages}
